Qutrit ZX-calculus is Complete for Stabilizer Quantum Mechanics

In this paper, we show that a qutrit version of ZX-calculus, with rules significantly different from that of the qubit version, is complete for pure qutrit stabilizer quantum mechanics, where state preparations and measurements are based on the three dimensional computational basis, and unitary operations are required to be in the generalized Clifford group. This means that any equation of diagrams that holds true under the standard interpretation in Hilbert spaces can be derived diagrammatically. In contrast to the qubit case, the situation here is more complicated due to the richer structure of this qutrit ZX-calculus.

==> eptcsdata.tex <==
\providecommand{\firstpage}{58}
\providecommand{\publicationstatus}{Bob Coecke and Aleks Kissinger (Eds.):\\ 14th International Conference on Quantum Physics and Logic (QPL)\\
EPTCS 266, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.266.3}{10.4204/EPTCS.266.3}}
\pdfoutput=1

